On quantum superpositions of graphs, no-signalling and covariance

We provide a mathematically and conceptually robust notion of quantum superpositions of graphs. We argue that, crucially, quantum superpositions of graphs require node names for their correct alignment, which we demonstrate through a no-signalling argument. Nevertheless, node names are a fiducial construct, serving a similar purpose to the labelling of points through a choice of coordinates in continuous space. Graph renamings, aka isomorphisms, are understood as a change of coordinates on the graph and correspond to a natively discrete analogue of continuous diffeomorphisms. We postulate renaming invariance as a symmetry principle in discrete topology of similar weight to diffeomorphism invariance in the continuous. We explain how to impose renaming invariance at the level of quantum superpositions of graphs, in a way that still allows us to talk about an observable centred at a specific node.

==> macro_nodes_inline.tex <==
\usepackage[utf8]{inputenc}
\usepackage{tikz}
\usetikzlibrary{shapes.geometric}

%opening
\makeatletter
\tikzset{circle split part fill/.style  args={#1,#2}{%
 alias=tmp@name, % Jake's idea !!
  postaction={%
    insert path={
     \pgfextra{% 
     \pgfpointdiff{\pgfpointanchor{\pgf@node@name}{center}}%
                  {\pgfpointanchor{\pgf@node@name}{east}}%            
     \pgfmathsetmacro\insiderad{\pgf@x}
      %\begin{scope}[on background layer]
      %\fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
      %                    (0:180:\insiderad-0.5\pgflinewidth)--cycle;
      %\fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
      %                     (180:360:\insiderad-0.5\pgflinewidth)--cycle;  
      \fill[#1] (\pgf@node@name.base) ([xshift=-\pgflinewidth]\pgf@node@name.east) arc
                          (0:180:\insiderad-\pgflinewidth)--cycle;
      \fill[#2] (\pgf@node@name.base) ([xshift=\pgflinewidth]\pgf@node@name.west)  arc
                           (180:360:\insiderad-\pgflinewidth)--cycle;            %  \end{scope}   
         }}}}}  
 \makeatother
\newcommand{\splittednode}[2]{\resizebox{20pt}{10pt}{
\tikz{
\draw (-0.3,0)node[above]{\scriptsize :$a$}--(+0.3,0)node[above]{\scriptsize :$b$};
\node[draw,rotate=90, circle, circle split part fill={#1,#2}]{};
}}}

\newcommand{\edgynode}[2]{\resizebox{30pt}{10pt}{
\tikz{
\draw (0,0)--(1,0);
\node[draw,minimum size=1 pt,rotate=270,semicircle,fill=#1]{}; \node[draw,minimum size=1 pt,rotate=90,semicircle,fill=#2]at (1,0){};
}
}}

\newcommand{\lineoffour}[8]{\makebox{
\tikz{
\draw (-0.3,0)--(3.3,0);
\node[] at (-0.7,0) {\dots};
\node[draw,rotate=90, circle, circle split part fill={#1,#2}]{};
\node[] at (0,-0.3) {$u$};
\draw (-0.3,0)node[above]{\scriptsize :$a$} (+0.3,0)node[above]{\scriptsize :$b$};

\node[draw,rotate=90, circle, circle split part fill={#3,#4}]at (1,0){};
\node[] at (1,-0.3) {$v$};
\draw (0.7,0)node[above]{\scriptsize :$a$} (+1.3,0)node[above]{\scriptsize :$b$};

\node[draw,rotate=90, circle, circle split part fill={#5,#6}]at (2,0){};
\node[] at (2,-0.3) {$w$};
\draw (1.7,0)node[above]{\scriptsize :$a$} (+2.3,0)node[above]{\scriptsize :$b$};

\node[draw,rotate=90, circle, circle split part fill={#7,#8}]at (3,0){};
\node[] at (3,-0.3) {$x$};
\draw (2.7,0)node[above]{\scriptsize :$a$} (+3.3,0)node[above]{\scriptsize :$b$};
\node[] at (3.8,0) {\dots}
}}
}

\newcommand{\lineoffourmodulo}[8]{\makebox{
\tikz{
\draw (-0.3,0)--(3.3,0);
\node[] at (-0.7,0) {\dots};
\node[draw,rotate=90, circle, circle split part fill={#1,#2}]{};
\draw (-0.3,0)node[above]{\scriptsize :$a$} (+0.3,0)node[above]{\scriptsize :$b$};

\node[draw,rotate=90, circle, circle split part fill={#3,#4}]at (1,0){};
\draw (0.7,0)node[above]{\scriptsize :$a$} (+1.3,0)node[above]{\scriptsize :$b$};

\node[draw,rotate=90, circle, circle split part fill={#5,#6}]at (2,0){};
\draw (1.7,0)node[above]{\scriptsize :$a$} (+2.3,0)node[above]{\scriptsize :$b$};

\node[draw,rotate=90, circle, circle split part fill={#7,#8}]at (3,0){};
\draw (2.7,0)node[above]{\scriptsize :$a$} (+3.3,0)node[above]{\scriptsize :$b$};
\node[] at (3.8,0) {\dots}
}}
}
